HierFlow: Hierarchical Coupled Dual-Space Search for Automatic Agentic Workflow Generation

Although structured workflows empower Large Language Models (LLMs) to tackle complex problems, automating their creation is severely hindered by a vast combinatorial search space, frequently resulting in inflexible and resource-heavy offline training dependencies. To address this, we conceptualize workflow generation as an intertwined topology-and-execution search paradigm, where the broader topological layer dictates subtask boundaries and lower-level execution outcomes actively reshape the topology itself. Building on this foundation, we introduce HierFlow, a training-free, test-time hierarchical search architecture that automates agentic workflow design by merging feedback-guided topology adjustments with a fast, MCTS-inspired tree search for sub-workflow optimization. HierFlow maximizes efficiency through an intelligent gating module that selectively triggers execution-level searches based on contextual necessity, a mechanism we further support with an in-depth analysis detailing how varying degrees of cross-task coupling impact the effectiveness of hierarchical splitting. Comprehensive testing across question answering, mathematical reasoning, and code generation benchmarks confirms that HierFlow consistently outperforms strong baselines, delivering an optimal balance of high-quality results and computational efficiency without any additional training overhead.

==> sections/related.tex <==

% \subsection{Handcrafted Agentic Workflows}

% Early agentic reasoning methods predominantly rely on handcrafted workflows, where the reasoning structure and execution procedure are manually specified and fixed at inference time. 
% % Chain-of-Thought (CoT)~\cite{CoT} prompting introduces a linear reasoning workflow with explicitly defined intermediate steps, while Self-Consistency~\cite{CoTSC} improves robustness by sampling and aggregating multiple reasoning paths under the same fixed workflow. Self-Refine~\cite{SR} further adopts a predefined iterative refinement loop, enabling the model to critique and revise its outputs across multiple rounds. LLM-Debate~\cite{llmdebate} extends handcrafted workflows to multi-agent settings by explicitly designing agent roles and interaction protocols. 
% Representative examples include Chain-of-Thought (CoT)~\cite{CoT}, Self-Consistency~\cite{CoTSC}, Self-Refine~\cite{SR}, and LLM-Debate~\cite{llmdebate}.
% Despite their effectiveness, these methods share a common limitation: the workflow structure is manually designed and remains static, limiting adaptability as task complexity increases.
\label{sec:related}

\noindent \textbf{Workflow Representation via Proxy Spaces.} Since direct search over the workflow space is highly challenging, existing approaches typically reformulate workflow generation by introducing a proxy space, in which searching over proxy representations serves as a surrogate for searching over workflows themselves~\cite{survey}. A key property of a proxy space is that each proxy instance induces a valid workflow, enabling indirect optimization over the workflow space. Depending on the specific form of the proxy, existing methods commonly operate in natural language (NL) program~\cite{autoflow}, code~\cite{aflow}, topology~\cite{flow}, or handcrafted spaces~\cite{dyflow}, which offer different trade-offs between expressiveness and tractability. 
NL proxies are highly expressive but excessively redundant and thus difficult to search; code proxies provide more structured representations but remain complex due to execution-level combinatorics; topology proxies abstract away execution details, yielding a smaller but less expressive space suitable for coarse-grained pruning; and handcrafted proxies further restrict the space to improve tractability at the cost of flexibility.

\begin{wraptable}{r}{0.55\textwidth}
\caption{Comparison between automatic agentic workflow generation methods. FD stands for ``Feedback-Driven''. For HierFlow, ``coupled'' denotes bidirectional topology--execution updates rather than a fixed pipeline over two spaces.}
    \label{tab:comparison}
    \footnotesize
    \centering
    
    \setlength\tabcolsep{3.5pt}
    
    \begin{tabular}{lccccc}
        \toprule
        \toprule


        Method & Scope & FD & Search Space & Primary Cost\\

        \midrule

        ADAS & Task-Level & \textcolor{red}{\ding{55}} & Code & Offline Search \\

        AutoFlow & Task-Level & \textcolor{red}{\ding{55}} & NL Program & Offline Search \\

        AFlow & Task-Level & \textcolor{red}{\ding{55}} & Code & Offline Search \\

        MaAS & Query-Level & \textcolor{red}{\ding{55}} & Handcrafted & Offline Training \\

        DyFlow & Query-Level & \textcolor{green}{\ding{51}} & Handcrafted & Offline Training \\

        Flow & Query-Level & \textcolor{green}{\ding{51}} & Topology & Orchestration \\

        \midrule

        \sysname{} & \multirow{2}{*}{Query-Level} & \multirow{2}{*}{\textcolor{green}{\ding{51}}} & Coupled \& & Test-Time \\

        (Ours)& & & Topology--Code & Scaling \\

    
        \bottomrule
        \bottomrule
    \end{tabular}
    
\end{wraptable}

\label{sec:method}

\begin{figure*}[t]
    \centering
    % \setlength{\belowcaptionskip}{-4pt}
    \includegraphics[width=\linewidth]{figures/overall.pdf}
    \caption{
    Illustrative example of how \sysname{} operates at inference time.
Given a query, \sysname{} first performs \textbf{(a) initialization} by identifying an initial structure in the topology space, where each node represents a subtask and corresponds to a sub-space of the overall workflow space. Based on this structure, (\textbf{b) upper-level search} is conducted to evaluate whether the current structure requires refinement, with a gating mechanism jointly determining whether any subtask should be activated for \textbf{(c) lower-level search}, which applies a lightweight MCTS to explore a sub-workflow in the corresponding code space. The key distinction is the closed-loop coupling: topology determines the subtask-level code-search domains, while execution feedback can trigger topology repair and rewinding. See Section~\ref{sec:method} for more details.
    }
    \label{fig:overall}
\end{figure*}


\noindent \textbf{Automatic Agentic Workflow Generation.} Recent methods automate workflow generation by formulating it as a search-based optimization problem over a proxy space. Based on the scope of generated workflow, they can be categorised into task-level (\textit{i.e.} dataset-level) and query-level approaches. Task-level methods aim to discover a general workflow for a given task or dataset, typically through offline search in code (\textit{e.g.,} ADAS~\cite{adas} and AFlow~\cite{aflow}) or NL program spaces (\textit{e.g.,} AutoFlow~\cite{autoflow}). In contrast, query-level methods generate workflows tailored to individual queries to improve generalisation. Representative examples include MaAS~\cite{maas}, which learns to select from predefined architectures, and feedback-driven approaches such as DyFlow~\cite{dyflow} and Flow~\cite{flow}, which dynamically adjust workflows during execution.

Despite their effectiveness, existing methods remain limited in terms of generalization and training cost. Task-level methods are constrained by the training domain distribution and often fail to generalize to unseen domains. Among query-level methods, AFlow and MaAS require pre-constructed training datasets, leading to high training costs and similarly limiting their generalization. Flow avoids training and is thus task-agnostic, but does not explicitly address execution-level correctness. Moreover, these methods typically operate within a single proxy space, overlooking the complementary strengths of different spaces and the potential benefits of jointly leveraging them. 
% Inspired by these observations, we propose \sysname{}, a test-time scaling dual-space search approach for automatic agentic workflow generation.
We propose \sysname{} to address these limitations, with a comparison summarized in Table~\ref{tab:comparison}.





